Why is parameter averaging beneficial in SGD? An objective smoothing perspective

It is often observed that stochastic gradient descent (SGD) and its variants implicitly select a solution with good generalization performance; such implicit bias is often characterized in terms of the sharpness of the minima. Kleinberg et al. (2018) connected this bias with the smoothing effect of SGD which eliminates sharp local minima by the convolution using the stochastic gradient noise. We follow this line of research and study the commonly-used averaged SGD algorithm, which has been empirically observed in Izmailov et al. (2018) to prefer a flat minimum and therefore achieves better generalization. We prove that in certain problem settings, averaged SGD can efficiently optimize the smoothed objective which avoids sharp local minima. In experiments, we verify our theory and show that parameter averaging with an appropriate step size indeed leads to significant improvement in the performance of SGD.

==> archive/main_body_copy.tex <==
\section{Preliminary}
An alternative view \citep{kleinberg2018alternative} of the stochastic gradient descent (SGD) is the key in our analysis to relate to an implicit bias towards a flat minimum. We introduce this view with a convergence analysis and discuss the bias and optimization tradeoff caused by the step-size.
%In this paper we study the stochastic gradient descent (SGD) and its averaging scheme for the nonconvex optimization problems which include empirical and expected risk minimization problems. We first introduce SGD and its alternative view  of SGD which relates to optimization for the smoothed objective by stochastic noise.

\subsection{Stochastic Gradient Descent}
We consider risk minimization problems typically appearing in machine learning. 
Let $\ell(w,z)$ be a loss function consisting of the hypothesis function parameterized by $w \in \bR^d$ and a data example $z \in \bR^p$. 
Let $\mu$ be a data distribution over the data space $\bR^p$ and $Z$ be a random variable following $\mu$. Then, the objective function, which is nonconvex in general, is defined by 
\[ f(w) = \bE_{Z \sim \mu}[ \ell(w,Z)]. \]

Note that $f$ can represent both empirical and expected risks by setting $\mu$ to empirical and expected distributions, respectively. 
Moreover, we can further include the $\ell_2$-regularization in the objective $f$ and the perturbation by the data augmentation in the distribution $\mu$.

Given i.i.d. random variables $\{Z_{t+1}\}_{t=0}^\infty$ with the same distribution as $Z$, a stochastic gradient descent, randomly initialized at $w_0$, for optimizing $f$ is described as follows: for $t = 0, 1, 2, \ldots$
\begin{equation}\label{eq:sgd}
    w_{t+1} = w_t - \eta \left( \nabla f (w_t) + \epsilon_{t+1}(w_t) \right), 
\end{equation}
where $\eta > 0$ is the step-size and $\epsilon_{t+1}: \bR^d \rightarrow \bR^d$ is a random field representing the stochastic gradient noise with $Z_{t+1}$, i.e., for any $w \in \bR^d$, 
$\epsilon_{t+1}(w) = \nabla_w \ell(w, Z_{t+1}) - \nabla f(w)$.
That is, $\{ \epsilon_{t+1}(w)\}_{t=0}^\infty$ is a collection of i.i.d. zero-mean random variables taking values in $\bR^d$. 

%\begin{example}[Risk Minimization]\label{example:risk_mimimization}
%Let $\ell(w,z)$ be a loss function where $theta$ is a parameter of the hypothesis function and $z$ is a data example. Let $\mu$ be an empirical / true data distribution over the data space %and $Z$ be a random variable following $\mu$. Then, the empirical / expected risk is defined by 
%\[ f(w) = \bE_{Z \sim \mu}[ \ell(w,Z)]. \]
%Given i.i.d. random variables $\{Z_{t+1}\}_{t=0}^\infty$ with the same distribution as $Z$, the (standard) stochastic gradient at $t$-th iterate $w_t$ is defined as $\nabla_w \ell( w_t, Z_{t+1})$.
%In this setting, the stochastic noise $\epsilon_{t+1}$ can be $\epsilon_{t+1}(w) = \nabla_w \ell(w, Z_{t+1}) - \nabla f(w)$. % and $\cF_{t+1}$ can be a $\sigma$-algebra generated by $w_0, Z_1, Z_2, \ldots,Z_t$.
%Note that we can further include the $\ell_2$-regularization in the objective $f$ and the perturbation by the data augmentation in the distribution $\mu$.
%\end{example}

\subsection{Alternative View of Stochastic Gradient Descent}\label{subsec:alt_view}
We explain an alternative view of the stochastic gradient descent introduced in \cite{kleinberg2018alternative} which considers an associated iterations $\{v_t\}_{t=0}^\infty$ with $\{w_t\}_{t=0}^\infty$ and shows this iterations minimizes a smoothed objective function by the stochastic noise. We here define $v_t$ as a parameter obtained by the exact gradient descent from $w_t$, that is, $v_t = w_t - \eta \nabla f(w_t)$ and we analyze the update of $v_t$ instead of $w_t$. 
Using $w_{t+1} = v_t - \eta \epsilon_{t+1}(w_t)$, we get $v_{t+1} = v_t - \eta \epsilon_{t+1}(w_t) - \eta \nabla f( v_t - \eta \epsilon_{t+1}(w_t) )$.
Under a specific setting given later, $w \mapsto v=w - \eta \nabla f(w)$ becomes a smooth invertible injection and its inverse is differentiable, thus, we identify $\epsilon'_{t+1}(v)$ with $\epsilon_{t+1}(w)$ through the map $w\mapsto v$.
For the detail, see Appendix \ref{subsec:proof_sgd}
That is, we get an associated update rule of $v_t$ with $w_t$:
\begin{equation}\label{eq:implicit_sgd}
v_{t+1} = v_t - \eta \epsilon'_{t+1}(v_t) - \eta \nabla f( v_t - \eta \epsilon'_{t+1}(v_t) ).
\end{equation}
For the convenience, we refer to the rule (\ref{eq:implicit_sgd}) as an {\it implicit stochastic gradient descent}.
%Moreover, the equation: $\bE[v_{t+1} | \cF_t] = v_t - \eta \bE[\nabla f( v_t - \eta \epsilon'_{t+1}(v_t) ) | \cF_t]$ leads us to expect that the implicit stochastic gradient descent minimizes the following smoothed objective function:
Since, the conditional expectation of $\epsilon_{t+1}'(v_t)$ at $v_t$ is zero, we expect that the implicit stochastic gradient descent minimizes the following smoothed objective function:
\begin{equation}\label{eq:smoothed_objective}
    F(v) = \bE[ f( v - \eta \epsilon'(v)) ],
\end{equation}
where $\epsilon'$ is an independent copy of $\epsilon'_1$.
However, we note that implicit stochastic gradient descent is not a normal SGD because $\nabla f( v_t - \eta \epsilon'_{t+1}(v_t) )$ is a biased estimate of $\nabla F(v)$ in general\footnote{Let $(\Omega, \cF, P)$ be a probability space such that $\epsilon'(v)$ can be represented as a measurable map $\omega \in \Omega \mapsto \epsilon'(v,\omega)$. Then, $F(v) = \bE[f( v - \eta \epsilon'(v))] = \int f( v - \eta \epsilon'(v,\omega)) \rmd P(\omega)$ and $\nabla F(v) = \bE[\nabla (f( v - \eta \epsilon'(v)))] = \int \nabla (f( v - \eta \epsilon'(v,\omega))) \rmd P(\omega)$, whereas $\nabla f( v - \eta \epsilon'(v) )$ in Eq.~(\ref{eq:implicit_sgd}) means $\nabla f(w)|_{w= v - \eta \epsilon'(v)}$ which does not involve the derivative of $\epsilon'(v)$. 
Therefore, $\nabla F(v) \neq \bE[\nabla f( v - \eta \epsilon'(v) )]$ in general.}.

Indeed, the function (\ref{eq:smoothed_objective}) is a smoothed function of $f$ by the convolution with the noise $\eta \epsilon'$ and the level of smoothness is controlled by the step-size $\eta$ as seen in Figure \ref{fig:smoothed_objectives} which depicts how a nonconvex function (left figure, $\eta=0$) is smoothened and its sharp local minima are eliminated by an appropriately large step-size (right figure, $\eta=0.5$). Hence, we expect stochastic gradient descent can avoid sharp minima and tend to a flat minimum.
Moreover, by taking Taylor expansion of $f$, we see that $F(v)$ is an approximation of the function $f(v)$ plus the penalization on the high (positive) curvature of $f$ along the noise direction in expectation:
\begin{equation}\label{eq:regularized_objective}
    F(v) 
    %&= \bE[ f( v ) - \eta \nabla f(v)^\top \epsilon'(v)) + \frac{\eta^2}{2} \epsilon'(v)^\top \nabla^2 f(v) \epsilon'(v) + O(\eta^3)] \\
    = f(v) + \frac{\eta^2}{2} \Tr\left(\nabla^2 f(v) \bE[\epsilon'(v) \epsilon'(v)^\top]\right) + O(\eta^3).
\end{equation}

From the above observation, it is reasonable to impose some sort of convexity conditions at the solution of the smoothed objective $\cL(v)$ rather than the original objective $f(w)$. % which can be highly complex.
In this paper, we make the following assumptions to show the convergence of $F(v_t)$. 
Let $v_* = \argmin_{v \in \bR^d} F(v)$.
We note that $F$ and $v_*$ depend on the value of $\eta$, but we do not explicitly denote this dependency for simplicity.

\begin{assumption}\label{assump:sgd}\ 
\begin{description}[topsep=0mm,itemsep=0mm]%,itemindent=-12mm]
\item{{\bf(A1)}} $f: \bR^d \rightarrow \bR$ is nonnegative, twice continuously differentiable, and its Hessian is bounded, i.e., there is a constant $L>0$ such that for any $w \in \bR^d$, $-LI \preceq \nabla^2 f(w) \preceq LI$.
\item{{\bf(A2)}} There is a constant $c>0$ such that for any $v \in \bR^d$, $\nabla F(v)^\top (v-v_*) \geq c \|v-v_*\|^2$.
\item{{\bf(A3)}} There are $\sigma_1, \sigma_2 > 0$ such that for any $w \in \bR^d$, $\bE[ \|\epsilon_{t+1}(w)\|^2 | ] \leq \sigma_1^2$, $\bE[\|J_{\epsilon_{t+1}}^\top (w) \|_2 ] \leq \sigma_2$, where $J_{\epsilon_{t+1}}(w)$ is Jacobian of $\epsilon_{t+1}$. %\footnote{That is $J_{\epsilon_{t+1}}(w) = ( \partial \epsilon_{t+1,i}(w) /\partial w_j )_{i,j=1}^d$.}.
\end{description}
\end{assumption}

@ Explain Example \ref{example:risk_mimimization} satisfies the above conditions.
\cite{kleinberg2018alternative} empirically observed that deep neural networks satisfy A3.

The assumption *** differs from \cite{kleinberg2018alternative} which assumes the one point strong convexity centered at the solution to show the convergence of parameter $v_t$.

We adopt different proof strategy which allows for larger step size.

\begin{proposition}\label{prop:sgd}
Under Assumption {\bf (A1)}, {\bf (A2)}, {\bf (A3)}, run the stochastic gradient descent with $T$-iterations with the step size $\eta \leq \frac{1}{2L}$, then the implicit SGD satisfies the following inequalities:
\begin{align*}
    \frac{1}{T+1}\sum_{t=0}^T \bE[\|  v_t - v_* \|^2]
    &= O\left(T^{-1}\right) + \frac{2\eta\sigma_1^2}{c} + \frac{8\eta^2 \sigma_1^2 L}{3c} \left(1 + \frac{2 \eta \sigma_2^2}{c} \right), \\
    \left\| \frac{1}{T+1}\bE\left[ \sum_{t=0}^T \nabla F(v_t) \right] \right\|    
    &= \frac{4}{\sqrt{3}} \eta^{\frac{3}{2}} \sigma_1 \sigma_2 L^{\frac{1}{2}} + O\left( T^{-\frac{1}{2}} \right).
\end{align*}
\end{proposition}

The first inequality of Proposition \ref{prop:sgd} means that $v_t$ oscillates at distance $\sigma_1 \sqrt{ \frac{2\eta}{c} + \frac{8\eta^2L}{3c} \left(1 + \frac{2 \eta \sigma_2^2}{c} \right) }$ from $v_*$ in the final phase of training in expectation.
\AN{Discussion about the order of $\eta$,  $\sigma_1$. The meaning of the latter inequality. $w_t - v_* \sim v_t - v_* \sim O(\eta)$ because of $w_t - v_t \sim O(\eta)$.} 
Remarkably, this proposition shows the convergence of SGD to the minimum of the smoothed objective $F$ (\ref{eq:smoothed_objective}) by $O(\eta)$ as long as $F$ satisfies required assumptions even when local minima of the original objective $f$ exist. Thus, convergence to a flatter region is expected through an explicit expression as a regularized objective (\ref{eq:regularized_objective}).

\section{Averaged SGD with Large Step-size}
In this section, we show the averaged SGD can get closer to $v_*$ than SGD under certain settings.
In the averaged SGD, we run normal SGD (\ref{eq:sgd}) and take the average as follows:
\[ \overline{w}_{T+1} = \frac{1}{T+1}\sum_{t=1}^{T+1} w_t. \]
\cite{izmailov2018averaging} empirically demonstrated that averaged SGD converges to a flat region and achieves better generalization even when SGD oscillates with relatively large step size.
We theoretically attribute this phenomenon to that the limit of $\overline{w}_T$ can be closer to $v_*$ than $w_t, v_t$ under certain conditions by clarifying the dependency of the limit on the step size $\eta$.

Preferably, the implicit SGD (\ref{eq:implicit_sgd}) is more useful in analyzing the averaged SGD because the average $\overline{v}_T=\frac{1}{T}\sum_{t=0}^T v_t$ is consistent with $\overline{w}_T$ as confirmed below.
By the definition, we see 
\[ \overline{w}_{T+1} = \overline{v}_T + \frac{1}{T+1}\sum_{t=0}^{T}\epsilon_{t+1}(w_t), \]
where the noise term $\nicefrac{\sum_{t=0}^{T}\epsilon_{t+1}(w_t)}{(T+1)}$ is zero in expectation and its variance is upper bounded by $\nicefrac{\sigma_1^2}{(T+1)}$ under Assumption {\bf (A3)}. Hence, $\overline{w}_{T+1} - \overline{v}_{T}$ converges to zero in probability by Chebyshev's inequality: for any $r>0$, $\bP[ \|\overline{w}_{T+1} - \overline{v}_{T}\| > r ] \leq \nicefrac{\sigma_1^2}{(T+1)r^2} \rightarrow 0$ as $T \rightarrow \infty$, and the analysis of $\lim_{T\rightarrow \infty} \overline{w}_{T+1}$ reduces to that of $\lim_{T\rightarrow \infty} \overline{v}_T$.

We further make the additional assumptions on the smoothed objective $F: \bR^d \rightarrow \bR$.
\begin{assumption}\label{assump:asgd}\ 
\begin{description}[topsep=0mm,itemsep=0mm]%,itemindent=-12mm]
\item{{\bf(A4)}} $F$ is three times continuously differentiable and $\nabla^3 F$ is uniformly bounded, i.e., there is $M>0$ such that for any $v, w \in \bR^d$ and $k\in \{1,2,\ldots,\}$, $\| \nabla^3 F(v)ww^\top \| \leq 2 M \|w\|^2$, where $\nabla^3 F(v)ww^\top$ is a vector whose $k$-th element is $\sum_{i,j=1}^d \frac{\partial^3 F(v)}{\partial v_i \partial v_j} w_iw'_j$. %$k\in \{1,2,\ldots,\}$, $| \sum_{i,j=1}^d \frac{\partial^3 F(v)}{\partial v_i \partial v_j \partial v_k} v'_i v'_j | \leq M \|v'\|^2$. 
\item{{\bf(A5)}} $\nabla^2 F(v_*)$ is positive, i.e., there is $\mu > 0$ such that $\nabla^2 F(v_*) \succeq \mu I$.
\end{description}
\end{assumption}

\begin{proposition}\label{prop:asgd}
\begin{equation*}
    \| \bE[\overline{v}_T ]- v_* \| 
    \leq O\left( T^{-\frac{1}{2}} \right) + \frac{4}{\sqrt{3}\mu} \eta^{\frac{3}{2}} \sigma_1 \sigma_2 L^{\frac{1}{2}}
    +\frac{2\eta\sigma_1^2 M}{c \mu} + \frac{8\eta^2 \sigma_1^2 L M}{3c \mu} \left(1 + \frac{2 \eta \sigma_2^2}{c} \right).
\end{equation*}
\end{proposition}
\begin{proof}
We apply Taylor's theorem to $\nabla F$ around $v_*$ and obtain $\nabla F(v_t) = \nabla^2 F(v_*) (v_t - v_*) + R(v_t)$, where $R: \bR^d \rightarrow \bR^d$ satisfies $\| R(v) \| \leq M \|v-v_*\|^2$ by {\bf (A4)}. By taking average regarding $t\in \{0,1,\ldots,T\}$ and expectation, we get
\begin{equation*}
    \frac{1}{T+1}\bE\left[ \sum_{t=0}^T \nabla F(v_t) \right] = \nabla^2 F(v_*) ( \bE[\overline{v}_T] - v_*) + \frac{1}{T+1}\sum_{t=0}^T \bE[R(v_t)].
\end{equation*}
The left hand side and the last term can be bounded by Proposition \ref{prop:sgd}, which concludes the proof.
%\begin{equation*}
%    \mu \| \bE[\overline{v}_T ]- v_* \| 
%    \leq O\left( T^{-\frac{1}{2}} \right) + \frac{4}{\sqrt{3}} \eta^{\frac{3}{2}} \sigma_1 \sigma_2 L^{\frac{1}{2}}
%    +\frac{2\eta\sigma_1^2 M}{c} + \frac{8\eta^2 \sigma_1^2 L M}{3c} \left(1 + \frac{2 \eta \sigma_2^2}{c} \right).
%\end{equation*}
\end{proof}

\AN{Copy from introduction:} {\it Therefore, a better dependence of $O(\eta)$ than $O(\sqrt{\eta})$ means the high chance that the averaged SGD can achieve required optimization accuracy for the smoothed objective with larger step size than that SGD. For this argument to be theoretically valid, the required conditions (one point strong convexity at minimizer and regularity) should be satisfied uniformly for $0 < \forall \eta \leq \eta_0 (<1)$. Indeed, such a requirement certainly holds, for example, in a valley (see the top of Figure \ref{fig:alg_comparison}) and likely in the final phase of training deep neural network because the parameter finally falls in a valley (see the bottom of Figure \ref{fig:alg_comparison}).}

\section{Noise Injection}

\begin{figure}[t]
\center
\begin{minipage}[t]{0.3\linewidth}
\centering
\includegraphics[width=\textwidth]{figures/alg_comparison_nsgd0.png} 
\end{minipage} 
\begin{minipage}[t]{0.3\linewidth}
\centering
\includegraphics[width=\textwidth]{figures/alg_comparison_nsgd1.png} 
\end{minipage}
\caption{bbb}
\end{figure}
